Eight Ultra-faint Galaxy Candidates Discovered in Year Two of the Dark Energy Survey

We report the discovery of eight new ultra-faint dwarf galaxy candidates in the second year of optical imaging data from the Dark Energy Survey (DES). Six of these candidates are detected at high confidence, while two lower-confidence candidates are identified in regions of non-uniform survey coverage. The new stellar systems are found by three independent automated search techniques and are identified as overdensities of stars, consistent with the isochrone and luminosity function of an old and metal-poor simple stellar population. The new systems are faint (Mv > -4.7 mag) and span a range of physical sizes (17 pc < $r_{1/2}$ < 181 pc) and heliocentric distances (25 kpc < D < 214 kpc). All of the new systems have central surface brightnesses consistent with known ultra-faint dwarf galaxies (\mu < 27.5 mag arcsec$^{-2}$). Roughly half of the DES candidates are more distant, less luminous, and/or have lower surface brightnesses than previously known Milky Way satellite galaxies. Most of the candidates are found in the southern part of the DES footprint close to the Magellanic Clouds. We find that the DES data alone exclude (p < 0.001) a spatially isotropic distribution of Milky Way satellites and that the observed distribution can be well, though not uniquely, described by an association between several of the DES satellites and the Magellanic system. Our model predicts that the full sky may hold ~100 ultra-faint galaxies with physical properties comparable to the DES satellites and that 20-30% of these would be spatially associated with the Magellanic Clouds.

==> authors.tex <==

\author{
A.~Drlica-Wagner\altaffilmark{1,*},
K.~Bechtol\altaffilmark{2,3,\dagger},
E.~S.~Rykoff\altaffilmark{4,5},
E.~Luque\altaffilmark{6,7},
A.~Queiroz\altaffilmark{6,7},
Y.-Y.~Mao\altaffilmark{8,4,5},
R.~H.~Wechsler\altaffilmark{8,4,5},
J.~D.~Simon\altaffilmark{9},
B.~Santiago\altaffilmark{6,7},
B.~Yanny\altaffilmark{1},
E.~Balbinot\altaffilmark{10,7},
S.~Dodelson\altaffilmark{1,11},
A.~Fausti Neto\altaffilmark{7},
D.~J.~James\altaffilmark{12},
T.~S.~Li\altaffilmark{13},
M.~A.~G.~Maia\altaffilmark{7,14},
J.~L.~Marshall\altaffilmark{13},
A.~Pieres\altaffilmark{6,7},
K.~Stringer\altaffilmark{13},
A.~R.~Walker\altaffilmark{12},
T.~M.~C.~Abbott\altaffilmark{12},
F.~B.~Abdalla\altaffilmark{15,16},
S.~Allam\altaffilmark{1},
A.~Benoit-L{\'e}vy\altaffilmark{15},
G.~M.~Bernstein\altaffilmark{17},
E.~Bertin\altaffilmark{18,19},
D.~Brooks\altaffilmark{15},
E.~Buckley-Geer\altaffilmark{1},
D.~L.~Burke\altaffilmark{4,5},
A.~Carnero~Rosell\altaffilmark{7,14},
M.~Carrasco~Kind\altaffilmark{20,21},
J.~Carretero\altaffilmark{22,23},
M.~Crocce\altaffilmark{22},
L.~N.~da Costa\altaffilmark{7,14},
S.~Desai\altaffilmark{24,25},
H.~T.~Diehl\altaffilmark{1},
J.~P.~Dietrich\altaffilmark{24,25},
P.~Doel\altaffilmark{15},
T.~F.~Eifler\altaffilmark{17,26},
A.~E.~Evrard\altaffilmark{27,28},
D.~A.~Finley\altaffilmark{1},
B.~Flaugher\altaffilmark{1},
P.~Fosalba\altaffilmark{22},
J.~Frieman\altaffilmark{1,11},
E.~Gaztanaga\altaffilmark{22},
D.~W.~Gerdes\altaffilmark{28},
D.~Gruen\altaffilmark{29,30},
R.~A.~Gruendl\altaffilmark{20,21},
G.~Gutierrez\altaffilmark{1},
K.~Honscheid\altaffilmark{31,32},
K.~Kuehn\altaffilmark{33},
N.~Kuropatkin\altaffilmark{1},
O.~Lahav\altaffilmark{15},
P.~Martini\altaffilmark{31,34},
R.~Miquel\altaffilmark{35,23},
B.~Nord\altaffilmark{1},
R.~Ogando\altaffilmark{7,14},
A.~A.~Plazas\altaffilmark{26},
K.~Reil\altaffilmark{5},
A.~Roodman\altaffilmark{4,5},
M.~Sako\altaffilmark{17},
E.~Sanchez\altaffilmark{36},
V.~Scarpine\altaffilmark{1},
M.~Schubnell\altaffilmark{28},
I.~Sevilla-Noarbe\altaffilmark{36,20},
R.~C.~Smith\altaffilmark{12},
M.~Soares-Santos\altaffilmark{1},
F.~Sobreira\altaffilmark{1,7},
E.~Suchyta\altaffilmark{31,32},
M.~E.~C.~Swanson\altaffilmark{21},
G.~Tarle\altaffilmark{28},
D.~Tucker\altaffilmark{1},
V.~Vikram\altaffilmark{37},
W.~Wester\altaffilmark{1},
Y.~Zhang\altaffilmark{28},
J.~Zuntz\altaffilmark{38}
\\ \vspace{0.2cm} (The DES Collaboration) \\
}
\altaffiltext{*}{\href{mailto:kadrlica@fnal.gov}{kadrlica@fnal.gov}}
\altaffiltext{\textdagger}{\href{mailto:keith.bechtol@icecube.wisc.edu}{keith.bechtol@icecube.wisc.edu}}
 
\altaffiltext{1}{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\altaffiltext{2}{Wisconsin IceCube Particle Astrophysics Center (WIPAC), Madison, WI 53703, USA}
\altaffiltext{3}{Department of Physics, University of Wisconsin--Madison, Madison, WI 53706, USA}
\altaffiltext{4}{Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA}
\altaffiltext{5}{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}
\altaffiltext{6}{Instituto de F\'\i sica, UFRGS, Caixa Postal 15051, Porto Alegre, RS - 91501-970, Brazil}
\altaffiltext{7}{Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\altaffiltext{8}{Department of Physics, Stanford University, 382 Via Pueblo Mall, Stanford, CA 94305, USA}
\altaffiltext{9}{Carnegie Observatories, 813 Santa Barbara St., Pasadena, CA 91101, USA}
\altaffiltext{10}{Department of Physics, University of Surrey, Guildford GU2 7XH, UK}
\altaffiltext{11}{Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA}
\altaffiltext{12}{Cerro Tololo Inter-American Observatory, National Optical Astronomy Observatory, Casilla 603, La Serena, Chile}
\altaffiltext{13}{George P. and Cynthia Woods Mitchell Institute for Fundamental Physics and Astronomy, and Department of Physics and Astronomy, Texas A\&M University, College Station, TX 77843,  USA}
\altaffiltext{14}{Observat\'orio Nacional, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}
\altaffiltext{15}{Department of Physics \& Astronomy, University College London, Gower Street, London, WC1E 6BT, UK}
\altaffiltext{16}{Department of Physics and Electronics, Rhodes University, PO Box 94, Grahamstown, 6140, South Africa}
\altaffiltext{17}{Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA}
\altaffiltext{18}{CNRS, UMR 7095, Institut d'Astrophysique de Paris, F-75014, Paris, France}
\altaffiltext{19}{Sorbonne Universit\'es, UPMC Univ Paris 06, UMR 7095, Institut d'Astrophysique de Paris, F-75014, Paris, France}
\altaffiltext{20}{Department of Astronomy, University of Illinois, 1002 W. Green Street, Urbana, IL 61801, USA}
\altaffiltext{21}{National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA}
\altaffiltext{22}{Institut de Ci\`encies de l'Espai, IEEC-CSIC, Campus UAB, Carrer de Can Magrans, s/n,  08193 Bellaterra, Barcelona, Spain}
\altaffiltext{23}{Institut de F\'{\i}sica d'Altes Energies, Universitat Aut\`onoma de Barcelona, E-08193 Bellaterra, Barcelona, Spain}
\altaffiltext{24}{Excellence Cluster Universe, Boltzmannstr.\ 2, 85748 Garching, Germany}
\altaffiltext{25}{Faculty of Physics, Ludwig-Maximilians University, Scheinerstr. 1, 81679 Munich, Germany}
\altaffiltext{26}{Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Dr., Pasadena, CA 91109, USA}
\altaffiltext{27}{Department of Astronomy, University of Michigan, Ann Arbor, MI 48109, USA}
\altaffiltext{28}{Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA}
\altaffiltext{29}{Max Planck Institute for Extraterrestrial Physics, Giessenbachstrasse, 85748 Garching, Germany}
\altaffiltext{30}{Universit\"ats-Sternwarte, Fakult\"at f\"ur Physik, Ludwig-Maximilians Universit\"at M\"unchen, Scheinerstr. 1, 81679 M\"unchen, Germany}
\altaffiltext{31}{Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA}
\altaffiltext{32}{Department of Physics, The Ohio State University, Columbus, OH 43210, USA}
\altaffiltext{33}{Australian Astronomical Observatory, North Ryde, NSW 2113, Australia}
\altaffiltext{34}{Department of Astronomy, The Ohio State University, Columbus, OH 43210, USA}
\altaffiltext{35}{Instituci\'o Catalana de Recerca i Estudis Avan\c{c}ats, E-08010 Barcelona, Spain}
\altaffiltext{36}{Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain}
\altaffiltext{37}{Argonne National Laboratory, 9700 South Cass Avenue, Lemont, IL 60439, USA}
\altaffiltext{38}{Jodrell Bank Center for Astrophysics, School of Physics and Astronomy, University of Manchester, Oxford Road, Manchester, M13 9PL, UK}

